Chemically Aware Unitary Coupled Cluster with ab initio Calculations on System Model H1: A Refrigerant Chemicals Application

Circuit depth reduction is of critical importance for quantum chemistry simulations on current and near term quantum computers. This issue is tackled by introducing a chemically aware strategy for the Unitary Coupled Cluster ansatz. The objective is to use the chemical description of a system to aid in the synthesis of a quantum circuit. We combine this approach with two flavours of Symmetry Verification for the reduction of experimental noise. These method enable the use of System Model H1 for a 6-qubit QSE (Quantum Subspace Expansion). We present (i) calculations to obtain CH4 optical spectra; (ii) an atmospheric gas reaction simulation involving $[$CH$^{\cdot}_3$--H--OH$^{\cdot}]^{\ddagger}$. Using our chemically aware UCC state-preparation strategy in tandem with state of the art symmetry verification methods, we improve device yield for CH4 at 6-qubits. This is demonstrated by a 90% improvement in two-qubit gate count and reduction in relative error to 0.2% for electronic energy calculated on System Model H1.

==> declarations/disclosure.tex <==
Whilst this manuscript was being finalized, Ref. \cite{https://doi.org/10.48550/arxiv.2208.02414} appeared on the ArXiv showcasing excited-state properties computed on a superconducting quantum computer.
